Uncovering Limitations of Large Language Models in Information Seeking from Tables

Tables are recognized for their high information density and widespread usage, serving as essential sources of information. Seeking information from tables (TIS) is a crucial capability for Large Language Models (LLMs), serving as the foundation of knowledge-based Q&A systems. However, this field presently suffers from an absence of thorough and reliable evaluation. This paper introduces a more reliable benchmark for Table Information Seeking (TabIS). To avoid the unreliable evaluation caused by text similarity-based metrics, TabIS adopts a single-choice question format (with two options per question) instead of a text generation format. We establish an effective pipeline for generating options, ensuring their difficulty and quality. Experiments conducted on 12 LLMs reveal that while the performance of GPT-4-turbo is marginally satisfactory, both other proprietary and open-source models perform inadequately. Further analysis shows that LLMs exhibit a poor understanding of table structures, and struggle to balance between TIS performance and robustness against pseudo-relevant tables (common in retrieval-augmented systems). These findings uncover the limitations and potential challenges of LLMs in seeking information from tables. We release our data and code to facilitate further research in this field.

==> xxx-experiment.tex <==
\section{Experiments on TabIS}

In this section, we evaluate 12 representative LLMs on TabIS to answer the research question: \textit{Are LLMs \TODO{competent to perform TIS tasks} adequate to TIS tasks?}
\TODO{This research question is too broad, you should list some specific and interesting questions.}


\renewcommand{\arraystretch}{1.3} %控制行高
\begin{table*}[th]\centering
\setlength\tabcolsep{7pt}
\fontsize{10}{10}\selectfont
\begin{threeparttable}
\begin{tabular}{l|cccccc|c}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{TIS}} & \multicolumn{2}{c}{\textbf{TIS+TSU}} & \multicolumn{2}{c|}{\textbf{TIS+PRT}} & \multirow{2}{*}{\textbf{Avg.}} \\
\multicolumn{1}{l|}{}                                & \textbf{ToTTo}  & \textbf{HiTab} & \textbf{ToTTo}    & \textbf{HiTab}   & \textbf{ToTTo}    & \textbf{HiTab}    &                                \\ \hline
\textit{proprietary model}                          &                 &                &                   &                  &                   &                  &                                \\
Gemini-pro                                          & 85.6            & 66.6           & 81.3              & 65.1             & 79.4              & 64.8             & 73.8                           \\
GPT-3.5-turbo-instruct                              & 75.1            & 68.3           & 70.8              & 65.3             & 74.5              & 66.8             & 70.1                           \\
GPT-3.5-turbo-1106                                  & 72.1            & 57.5           & 66.8              & 50.4             & 66.7              & 53.0             & 61.1                           \\
GPT-3.5-turbo-16k                                   & 76.7            & 61.2           & 73.3              & 59.2             & 73.4              & 59.2             & 67.2                           \\
GPT-4-turbo-1106                                    & \textbf{91.2}   & \textbf{82.4}  & \textbf{90.0}     & \textbf{81.7}    & \textbf{89.7}     & \textbf{80.4}    & \textbf{85.9}                  \\
\midrule
\textit{open-source model}                          &                 &                &                   &                  &                   &                  &                                \\
Llama2-7b-chat                                      & 53.6            & 47.8           & 53.1              & 48.8             & 52.3              & 48.6             & 50.7                           \\
TableLlama-7b                                       & 54.3            & 47.7           & 54.1              & 47.8             & 54.1              & 47.9             & 51.0                           \\
Mistral-7b-instruct-v0.2                            & 73.2            & 56.9           & 69.9              & 53.5             & 68.8              & 57.1             & 63.2                           \\
Llama2-13b-chat                                     & 63.3            & 53.4           & 57.9              & 50.5             & 60.5              & 54.4             & 56.7                           \\
Mixtral-8*7b-instruct                               & 80.6            & 65.6           & 80.8              & \textbf{62.7}    & 76.2              & 57.9             & 70.6                           \\
Llama2-70b-chat                                     & 70.0            & 56.9           & 67.8              & 54.3             & 67.4              & 54.7             & 61.9                           \\
Tulu2-70b-DPO                                       & \textbf{85.7}   & \textbf{68.2}  & \textbf{81.9}     & 61.9             & \textbf{82.9}     & \textbf{64.0}    & \textbf{74.1}    \\
\bottomrule
\end{tabular}
\caption{Main results on TabIS. Random guess would achieve a 50\% accuracy.   Refer to Appendix x for more details.\label{tab:tis_main}}
\end{threeparttable}
\end{table*}


\subsection{Experimental Settings}

\noindent\textbf{Problem settings.}\quad  We evaluate LLMs in an open-domain table-based QA setting, where a linearized markdown table is presented in the context, and LLMs are required to answer a question given the context. All the questions are constructed into the binary-choice form, as detailed in Section \ref{tabis_bench}. We use one-shot example to familiarize the model with the task description and answering format, similar to previous work~\citep{tulu}.

We evaluate both proprietary and open-source LLMs. To enhance reproducibility, we set the temperature as 0 for proprietary models, and utilize the maximum probability of the first token as A or B to determine the outputs of open-source models.

\noindent\textbf{Proprietary models.}\quad 
We adopt three representative models:  \textbf{GPT-3.5}~\citep{chatgpt},  \textbf{GPT-4}~\citep{gpt4} and \textbf{Gemini-pro}~\citep{gemini-pro} .  GPTs\footnote{For GPTs, we investigate \textit{GPT-3.5-turbo-1106} and \textit{GPT-4-turbo-1106} for more consistent evaluation. We also report results on \textit{GPT-3.5-turbo-instruct} and \textit{GPT-3.5-turbo=16k}, since we find their performance varies greatly.} are a series of popular and capable LLM systems developed by OpenAI, with powerful textual understanding capabilities. Recent studies~\citep{numerical_reasoning,gpt4table,investigate_ttg} have shown great potential of these models on table-based understanding tasks. Gemini-pro\footnote{Gemini-pro is currently accessible via the \href{https://makersuite.google.com/app}{Gemini API}.} is one of Google's latest and most capable AI model which operates seamlessly across various modalities.

\noindent\textbf{Open-source models.}\quad 
Using proprietary LLM APIs as agents presents many challenges such as high costs and privacy concerns \citep{evaleval}. Therefore, we evaluate several popular open-source models: (1) \textbf{Llama2-chat}~\citep{llama2} ranging from 7b to 70b parameters; (2) \textbf{Mistral-7b-instruct-v0.2}~\citep{mistral-7b} and \textbf{Mixtral-8x7b-instruct}~\citep{mixtral-8*7b}, an instruction-tuned sparse mixture of experts language model; (3) \textbf{TableLlama-7b}~\citep{tablellama}, instruction-tuned from Llama2-7b, the first large generalist models for tables; and (4) \textbf{Tulu2-70b-DPO}~\citep{tulu2}, finetuned from Llama2-70b, the first 70b model aligned with DPO~\citep{dpo}. These models represent the highest-quality LLMs of different architectures and alignment strategies available to the community (though under restrictive licensing). 

\subsection{Main Results on TabIS}

We show exact-match scores of various models on the test set of TabIS in Table \ref{tab:tis_main}. We then analyze the performance of PIS and SIS respectively.

\noindent\textbf{PIS Performance.}\quad
Unexpectedly, despite PIS being straightforward for humans, all LLMs demonstrate subpar performance. The best performance of proprietary models and open-source models only achieve 66.1 (GPT-4) and 57.6 points (Tulu2-70b), respectively, while most models achieve near-random performance (50). 
Models do not consistently \TODO{excel} across all types of PIS tasks. Notably, the GPT series (GPT-4 and GPT-3.5) tend to perform better in column-oriented tasks (COL) relative to other tasks, whereas the Llama2 series (Llama2-7b, 13b, 70b) shows greater proficiency in cell-oriented tasks (CELL). This variation in performance could be attributed to the fact that models within the same series likely undergo similar pre-training and alignment processes, resulting in comparable inductive biases. \TODO{llama 看起来在各个方面表现的都不好} \TODO{Relative Cell/col/row上的表现呢?}

\noindent\textbf{SIS Performance.}\quad
Similar to PIS, proprietary models are generally more superior than open-source models, with the best average accuracy 85.7 (GPT-4) over 74.4 (Tulu2-70b). The overall SIS performance is much better than PIS, \TODO{partially due to their advanced textual understanding capabilities and alignment over table-based reasoning tasks}\TODO{为啥?}. 
Moreover, all models generally excel more in TTG than in HYB. HYB tasks, which only provide the location of highlighted cells as hints, are inherently more difficult than TTG tasks. However, models can refer to the cells contained in options to look back at the table to verify each option, therefore the performance drop is not dramatic.
In comparisons between datasets, all models show better performance on ToTTo than on HiTab, with improvements ranging from 5.8 to 19.0 points. This discrepancy is likely due to ToTTo predominantly featuring standard tables without merged cells, whereas HiTab includes tables with complex hierarchies, which pose greater challenges for tabular comprehension. \TODO{这一段太长了，要分几个要点}
Regarding the strategies for generating options (as illustrated in Figure \ref{fig:opt_strategy}), it has been observed that models tend to underperform with options generated through Human-Annotation and Exam-Judge. 
\TODO{这句话写在这里干啥？？}Human-annotation, while generally more difficult, also incurs higher costs. Our option generation pipeline strikes an effective balance between affordability and scalability.

\noindent\textbf{Alignment strategies matter.}\quad
A larger model size does not guarantee superior performance. Through more effective alignment strategies, a smaller model can outperform its larger counterparts within the same series. For instance, TableLlama, a version of Llama2-7b that has been instruction-tuned on a variety of table-based reasoning tasks, outperforms both the standard Llama2-7b and Llama2-13b models by 2.6 and 0.3 points, respectively. This underscores the effectiveness of instruction tuning specifically for table-based tasks in enhancing overall tabular comprehension.\TODO{加不加-chat?在PIS上表现好点，但是在SIS上的表现下降了啊？} Similarly, Tulu2-70b-DPO, which is fine-tuned from Llama2-70b for better adaptation, significantly improves upon Llama2-70b-chat's performance, achieving gains of 7.1 and 12.1 points on PIS and SIS tasks, respectively.\TODO{这个alignment到底是指什么？？？？ Tulu不是在 table上训练的吧？？}

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{tab_fig/opt_strategy.pdf}
\caption{Model performance in different option generation strategies. We average the accuracy of 12 LLMs of each strategy and dataset. Refer to Appendix x for more details.}
\label{fig:opt_strategy}
\end{figure}


\section{In-depth Analysis}

In this section, we conduct in-depth analysis to answer the research question: \textit{Can LLMs perform robustly on TIS tasks?}

\subsection{Effect of Target Locations on PIS}

Once humans understand the table structure and the task description, their PIS performance ideally remains consistent across various target locations. However, we find that LLMs work in a totally different manner. Specifically, we randomly sample 100 real tables with the same size (7 rows and 7 columns) and we ask the LLMs to perform PIS tasks on every possible locations of the table and report the accuracy on different locations. 

We show some results of RCL in Figure \ref{fig:evid_pos_heatmap}. Gemini-pro \TODO{为什么单选Gemini-pro呢？} exhibits large variance in different positions,with a disparity exceeding 30 points between its highest and lowest accuracy. On average, the data indicates that LLMs perform more effectively at the beginning (row 1, column 1) and ending (row 7, column 7) of tables. This pattern is likely influenced by the serialization of tables into one-dimension strings, rendering the middle part of the table more challenging to locate accurately. Similar patterns have been observed in other PIS tasks, as detailed in Appendix x.

\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{tab_fig/evid_pos_heat_map.pdf}
\caption{RCL performance with respect to target cell positions. We show a concrete example of Gemini-pro (left) and the averaged results of 12 models (right).}
\label{fig:evid_pos_heatmap}
\end{figure}

\noindent\textbf{No LLMs stand out in both robustness and performance.} We expand our analysis to include the calculation of the robustness score and mean performance for each model across six PIS tasks, illustrated in Figure \ref{fig:pis_pos_2d}. The robustness score for a task is determined by the standard deviation in accuracy across different target locations. Notably, the strongest LLM, GPT-4-turbo, exhibits the lowest stability. This highlights a common challenge among all LLMs, where achieving a balance between robustness and performance is difficult, with none excelling in both areas simultaneously.\TODO{这些结果都太奇怪了。。。}

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{tab_fig/pis_analysis.pdf}
\caption{PIS Robustness towards evidence locations and averaged accuracy for 12 models, tested and averaged on 6 PIS tasks.}
\label{fig:pis_pos_2d}
\end{figure}

\subsection{Effect of Cell Content on PIS}\label{sec:cell_content}

Logically, executing PIS tasks should not depend on the specific content of table cells, as this does not require an understanding of the table's semantics. Thus, the performance across tables with varying content should be consistent. To test this, we altered the cell contents in our PIS test set's real tables to random numbers (ranging from 1 to 8 digits) and random letters (also 1 to 8 characters in length), creating two new synthetic test sets named "letter" and "number."

However, we observe \textbf{significant variation in performance across different table contents}. As shown in Figure \ref{fig:pis_content}, the performance disparity between the test sets ranges from approximately 2.9 to 19.4 points. Intriguingly, GPT-4 shows markedly improved performance on the "number" set. This may be attributed to the activation of GPT-4's numerical processing capabilities, which are particularly relevant for PIS tasks (e.g. counting rows). This observation warrants further investigation in future studies.


\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{tab_fig/pis_content.pdf}
\caption{Accuracy on tables of different content, averaged on 6 PIS tasks.}
\label{fig:pis_content}
\end{figure}

\subsection{Effect of pseudo-relevant Tables on SIS}\label{sec:pseudo_relevant}

In real-world scenarios, LLM agents may be presented with additional context that, while superficially related to the "golden" table (the table that contains the answer), could be misleading and detrimentally affect their semantic information seeking capabilities~\citep{lost_in_the_middle}. We investigate the effects of adding pseudo-relevant tables, which appear relevant to the main table but are in fact non-essential. This situation frequently arises in retrieval-augmented LLM systems, where in response to a query, the system may retrieve several tables that are relevant to the query but not golden.
We construct a new test set based on our TTG test set. In particular, we prompt \textit{gpt-4-turbo-1106} to create one additional table mirroring the structure and headers of the golden table, yet contains varied data entries. Refer to Appendix x for more details.

We find that this setting \textbf{poses great challenge in balancing robustness and performance, especially for open-source models}. Specifically, to quantify a model's robustness, we measure the deviation between the accuracy without and with the pseudo-relevant table, averaged on ToTTo and HiTab. The results are shown in Figure \ref{fig:rag_scatter}. Notably, GPT-3.5-instruct and GPT-4-turbo emerged as both effective and robust. However, the two strongest open-source models, Tulu-70b and Mixtral-7b*8, exhibit the lowest robustness levels.


\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{tab_fig/rag_scatter.pdf}
\caption{SIS Robustness towards pseudo-relevant tables and averaged accuracy for 12 models, tested and averaged on ToTTo and HiTab.}
\label{fig:rag_scatter}
\end{figure}


\section{Improving Table Information Seeking}

In this section, we investigate the improvement of table information seeking via supervised finetuning over weakly-supervised datasets. 

We first utilize our proposed data generation pipeline (Section \ref{tabis_bench}) to construct weakly-supervised TIS training datasets. For PIS, we apply our templates over additional 15,000 collected tables (Section \ref{pis_dataset}). For SIS, we apply our option generation pipeline\footnote{Considering high cost of accessing GPT-4-turbo API, we use GPT-3.5-turbo-16k instead.} without manual checking. The statistics of the training dataset are shown in Table \ref{fig:dataset_example}.  We fully finetune \textit{Llama2-13b-chat} on this training set for 2 epochs (More training details in Appendix x) to obtain \textbf{TISLlama}. We evaluate TISLlama on held-in test set TabIS\footnote{Note that training on the weakly-supervised datasets may introduce the spurious correlation between the model-generated options and the wrong options. Thus we only evaluate on human-annotated samples for fair comparision.} and three held-out datasets used in our analysis: PIS-num (Section \ref{sec:cell_content}), PIS-letter (Section \ref{sec:cell_content}) and SIS-pr (Section \ref{sec:pseudo_relevant}).

As shown in Table \ref{tab:sft_held_in} and Table \ref{tab:sft_held_out}, TISLlama achieves significant improvement in both held-in and held-out evaluation, consistently improving about 20 points and 9 points on PIS and SIS tasks, respectively. Note that PIS can be regarded as a set of logical rules and is highly generalizable across tables. The consistent improvement on PIS tasks indicates that even though the PIS logic rules are not explicitly encoded in the LLMs, we can teach them to learn such rules by creating examples of the rules on a large scale. 
On the other hand, the SIS performance still lags behind larger models without specific finetuning. This indicates that SIS poses a greater challenge for LLMs, which calls for future investigations on this task.





\renewcommand{\arraystretch}{1.3} %控制行高
\begin{table}[th]\centering
\setlength\tabcolsep{3pt}
\fontsize{10}{10}\selectfont
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
\textbf{Model}   & \textbf{B-TIS} & \textbf{SU-TIS} & \textbf{M-TIS} & \textbf{Avg.} \\
\midrule
Llama2-13b-chat  & 56.8         & 53.3             & 56.5             & 55.5          \\
Llama2-70b-chat  & 58.2         & 58.1             & 58.5             & 58.3          \\
Tulu2-70b-DPO $~\clubsuit$    & 69.7         & 69.1             & 64.7             & 67.8          \\
GPT-4-turbo-1106 $\spadesuit$  & 81.2         & 77.4             & 79.1             & 79.2          \\
\midrule
% Llama2-7b-chat-SFT                   & 53.1          & 49.4            \\
TISLlama (ours)   & 73.3      & 73.7        & 72.7        & 73.2 \\
\bottomrule
\end{tabular}
\caption{In-domain evaluation of TISLlama on TabIS. $~\clubsuit$ and $\spadesuit$ denotes the best open-source model and proprietary model in our evaluation. \label{tab:sft_held_in}}
\end{threeparttable}
\end{table}


==> xxx-introduction-xxx.tex <==

\section{Introduction}

Tables are ubiquitous sources of rich information throughout the web and documents. Precisely seeking relevant information from tables is pivotal for a broad range of real-world applications, such as financial analysis, scientific research, and human resources management. Currently, Large language models (LLMs) \citep{gpt3, palm, gpt4, llama2, gemini-pro} have demonstrated remarkable superiority in seeking information from passages~\citep{lost_in_the_middle}. However, the effectiveness of LLMs in seeking information from tables remains underexplored.  

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{tab_fig/intro_eval_example.pdf}
\caption{(upper) A table-to-text generation example (simplified) of unreliable evaluation via surface-level metrics BLEU and ROUGE. Target cells are highlighted. (lower) Three levels of table information seeking.}
\label{fig:eval_example}
\end{figure}

\renewcommand{\arraystretch}{1.3} %控制行高
\begin{table*}[th]\centering
\setlength\tabcolsep{5pt}
\fontsize{10}{10}\selectfont
\begin{threeparttable}
\begin{tabular}{l|cccccc}
\toprule
\textbf{Dataset}   & \textbf{\# Train} & \textbf{\# Test} & \textbf{Annotation} & \textbf{SIS} & \textbf{PIS}  & \textbf{Reliable Evaluation} \\
\midrule
GPT4Table~\citep{gpt4table} & 0        & 6,000   & \ding{55}         & \ding{55}  & \ding{51}             & \ding{51}                 \\
LoTNLG~\citep{investigate_t2t}    & 0        & 4,305    & \ding{51}        & \ding{51} & \ding{55}              & \ding{55}                  \\
F2WTQ~\citep{investigate_t2t}     & 0        & 4,344    & \ding{51}        & \ding{51} & \ding{55}              & \ding{55}                  \\
TabIS (ours)     & 142,447   & 7,929    & \ding{51}    & \ding{51} & \ding{51}   & \ding{51}  \\          
\bottomrule
\end{tabular}
\caption{Comparison between TabIS and other tabular understanding benchmarks for LLMs. We only report the test set of table information seeking tasks in GPT4Table. \label{tab:compare_dataset}}
\end{threeparttable}
\end{table*}

Recent studies~\citep{invest_ttg,distill_table_reason} have highlighted the LLMs' superiority in faithfully seeking information from tables, utilizing the table-to-text generation task as a benchmark.  
However, their evaluations heavily rely on traditional surface-level metrics such as BLEU~\citep{bleu} and ROUGE~\citep{rouge}, or metrics based on model predictions such as NLI-Acc~\citep{nli_acc}. Since LLM responses can vary significantly in format from the golden references, utilizing these automated metrics might result in \textbf{unreliable evaluations}~\citep{parent}.
Figure \ref{fig:eval_example} illustrates this issue, where a finetuned model's incorrect description receives higher BLEU/ROUGE scores than GPT-3.5's output. This discrepancy likely arises because GPT-3.5, without finetuning on this specific dataset, may not replicate the reference's response style. 

% Moreover, prior research has not conducted a thorough investigation of table information seeking.  As shown in Figure \ref{fig:eval_example}, this capability could be broken down into two levels: perceptual information seeking (PIS) and semantic information seeking (SIS). PIS, which requires comprehension of table structures, is a fundamental capability in understanding the table semantics - to understand the meaning of a specific cell, one must first be aware of its contextual table structures (e.g. cells within the same row/column). While this may seem intuitive to humans, it can pose significant challenges for LLMs, especially since tables are presented to these models in a serialized format, like markdown or HTML. SIS requires an accurate understanding of table semantics and is highly related to table-to-text generation tasks.
% Previous research has mainly concentrated on SIS~\citep{invest_ttg}, largely overlooking PIS.

In this paper, we aim to \textbf{systematically} analyze TIS capabilities in a \textbf{reliable} manner. We create a more comprehensive benchmark for \textbf{Tab}le \textbf{I}nformation \textbf{S}eeking (TabIS), which contains large amount of training samples and high-quality test samples for both PIS and SIS, as shown in Figure \ref{tab:compare_dataset}. To ensure reliable assessment, this benchmark employs a single-choice question format (with two options per question), similar to popular LLM benchmarks such as MMLU~\citep{mmlu} and BBH~\citep{bbh}.

For PIS, TabIS investigates six probing tasks, involving lookup of table components based on absolute or relative positions. For SIS, TabIS investigate two probing tasks: Table-to-Text Generation (TTG) and its hybrid form with PIS (HYB) on two public datasets, ToTTo~\citep{totto} and Hitab~\citep{hitab}.
 We organize all samples of TabIS into the binary-choice form to overcome the unreliable evaluation challenge. 

We assess the performance of 12 representative LLMs (5 proprietary models and 7 open-source models) on TabIS and further investigate their TIS robustness towards three aspects: target locations (PIS), cell content (PIS) and pseudo-relevant tables (SIS). Our main findings uncover limitations of current LLMs in information seeking from tables: 
\begin{itemize}
    \item \textbf{LLMs achieve unsatisfying overall performance in both PIS and SIS tasks.} The best performance for PIS and SIS tasks is 66.1 and 85.7 points, respectively (random guess would be 50 points).
    \item \textbf{LLMs struggle to balance robustness\TODO{what is robustness} and overall performance, especially for open-source models.} For example, GPT-4-turbo achieves the best overall performance on PIS but exhibits the lowest robustness towards targe locations.
\end{itemize}

TabIS provides an objective, systematical and reproducible benchmark for evaluating LLMs in information seeking from tables. It underscores the limitations of current LLMs that have been neglected by previous studies. We hope this benchmark can foster future research in building table generalist models. 



==> xxx-tabis_bench-xxx.tex <==
\section{TabIS Benchmark}\label{tabis_bench}

We investigate the table information seeking capabilities of LLMs from three aspects: . To ensure a more objective assessment, the test samples in the benchmark have been meticulously organized into single-choice questions, each offering two options: A and B. 


\subsection{Perceptual Information Seeking}

Perceptual Information Seeking (PIS) refers to the capability of identifying and retrieving information from tables by understanding and \TODO{interacting} with their \TODO{spatial and visual} structure. This  necessitates to perceive the two-dimensional spatial layout inherent in tables, such as the positioning of cells, rows, and columns, to access desired content based on the location within the table space.  PIS is a critical skill in human comprehension of tables and is vital for effectively navigating and interpreting data arranged in a tabular format. \TODO{only use words like critical/vital can not show the importance of this task}

% Intuitively, the difficulty of the PIS task is highly dependent on the table size provided for each question. 

To examine the perceptual information seeking capability of large language models, we propose six probing tasks: positional cell lookup (PCL), relative cell lookup (RCL), positional row lookup (PRL), relative row lookup (RRL), positional column lookup (PLL), relative column lookup (RLL). These tasks require LLMs to acquire certain surface-level table components (cell, row and column) based on relative or absolute position information. We show an example of positional cell lookup (PCL) and relative cell lookup (RCL) in Figure \ref{fig:dataset_example}.\todo{maybe a taxonomy figure? clear}

\subsubsection{PIS Dataset Construction}\label{pis_dataset}

We generate samples for each task by applying predefined templates on high-quality tables. All question templates are shown in  Table \ref{tab:pis_template} in Appendix. We collect tables from four public datasets: WikiSQL~\citep{wikisql}, WikiTableQuestions~\citep{wikitablequestions}, HybridQA~\citep{hybridqa} and FeTaQA~\citep{fetaqa}. These tables are all semi-structured HTML tables collected from Wikipedia, spaning a wide array of topics such as sports and \TODO{countries}. After deduplicating these tables, we obtain a total of 49,561 high-quality tables. For the test set, we randomly sample 1\% tables and generate one sample per table for each PIS task.

For each sample, the options are generated by randomly sampling cells, rows and columns in proximity to the golden answer, employing a gaussian distribution $\mathcal{N}(\mathbf{p}, 1)$, where $\mathbf{p}$ denotes the position of the golden answer. \TODO{relative?}


\begin{figure*}[t]
\centering
\includegraphics[width=0.98\textwidth]{tab_fig/SIS_example.pdf}
\caption{Examples of TIS, TIS+TSU and pseudo-relevant tables. The TIS+TSU sample shares the same options and answer with the TIS sample. See Appendix x for more examples.}
\label{fig:dataset_example}
\end{figure*}

\subsection{Semantic Information Seeking}

Semantic Information Seeking (SIS) refers to the capability of uncovering meaningful and relevant insights in response to specific information requests or data inquiries from tables.\TODO{highlight the difference between PIS and SIS} By searching and describing table facts into natural language, LLMs can act as valuable assistants in aiding users with table comprehension and decision-making, liberating them from the need to comb through the whole complex table. 

We use the table-to-text generation (TTG) task and a hybrid combination of PIS and TTG (HYB) to investigate the SIS capability of LLMs. Given a table and a set of highlighted table cells, TTG aims at producing a one-sentence description about the cells. Similarly, HYB  aims at generating a description/insight based on some position information. Since the correct response can be quite different from the golden reference literally, we transform the two task into a binary-choice question for more objective and precise evaluation. One example of TTG and HYB are shown in Figure \ref{fig:dataset_example}.

We build our test benchmark upon two public datasets (detailed in Section \ref{sec:sis_data_const}). We take the golden reference as the answer and generate one wrong option for each TTG sample. The HYB samples are generated via replacing the cells with their approximate positions (e.g. row 5). In the following section, we introduce our option generation pipeline.


\subsubsection{SIS Option Generation Pipeline}\label{sec:sis_option_generation}
For each TTG sample $(T, C, R)$, where $T, C, R$ denotes the table, a set of highlighted cells\TODO{where is C in Figure1} and the golden reference. We aim to generate a challenging option $O$ to form an instance $(T,C,R,O)$. These instances are then utilized to assemble a multi-choice quiz in which, given one table $T$ and a set of cells $C$, models are tasked with selecting the correct option between $R$ and $O$. The option generation follows a three-step methodology:
\begin{enumerate}[itemsep=0pt, parsep=0pt, topsep=0pt, partopsep=0pt]
    \item For each TTG sample, we generate one challenging candidate option, expecting that the option is unfaithful to the table but is similar to the golden reference.
    \item Next, we perform adversarial filtering~\citep{evaleval} to \TODO{filter out} difficult candidate instances. We test three different models on two different presentation order of the options ($R, O$ and $O,R$) to obtain six predicted labels. And we retain the instances of which a majority of labels are wrong. 
    \item Finally, we conduct manual checking and modification over difficult instances to ensure objectivity and correctness.  
\end{enumerate}
We put more details of the option generation pipeline in appendix X. In the following, we introduce four option strategies used in step 1.

\noindent\textbf{Modify-Input (MI).}\quad   We directly prompt gpt-4 to first modify the highlighted cells 
$C$ slightly, resulting in a modified set $C'$, and subsequently perform the TTG task using $C'$ to produce an unfaithful statement $O$. 

\noindent\textbf{Modify-Output (MO).}\quad   We directly prompt gpt-4 to refer to the golden reference $R$ and make up a new statement that contains highlighted cells $C$, but is not faithful to the table fact. 

\noindent\textbf{Exam-Judge (EJ).}\quad Given the table $T$ and a set of cells $C$, we first instruct a weak LLM agent to perform the TTG task, yielding multiple candidate responses $O'$. Subsequently, a more advanced LLM agent\footnote{We use gpt-3.5-turbo-16k and gpt-4 as the weak and strong LLM agent, respectively.} is employed to identify responses that are unfaithful to the table. Among these, the one that is most literally similar to the golden reference $R$ is selected as the option. The underlying idea is to automatically obtain incorrect responses from relatively weak agents, thereby producing strong false options that are \TODO{less distinguishable}.

\noindent\textbf{Human-Annotation (HA).}\quad  Beyond the automated generation process, we also instruct annotators to revise the model-generated incorrect options during manual checking, ensuring the altered options are convincingly deceptive, making it difficult for individuals to recognize them as incorrect answers. \TODO{这个算是step1 还是step3?}

\subsubsection{SIS Dataset Construction}\label{sec:sis_data_const}
We generate our dataset using two public TTG datasets: (1) \textbf{ToTTo}~\citep{totto} is an open-domain English table-to-text dataset with over 120,000 examples. The tables are all semi-structured HTML tables from Wikipedia pages and the reference sentences are mainly descriptive statements over the table fact.
(2) \textbf{HiTab}~\citep{hitab} is a cross-domain hierarchical table dataset with over 10,000 samples, constructed from a wealth of statistical reports. It contains hierarchical tables and accompanied descriptive sentences collected from StatCan and NSF.  Compared to ToTTo, HiTab poses a greater challenge to table information seeking since the tables are with hierarchies and the sentences may involve numerical reasoning (e.g. comparison and simple computation).

\subsection{Dataset Statistics and Quality Assessment}

\renewcommand{\arraystretch}{1.4} %控制行高
\begin{table}[t]\centering
\setlength\tabcolsep{7pt}
\fontsize{10}{10}\selectfont
\begin{threeparttable}
\begin{tabular}{ll|cc}
\toprule
\multicolumn{2}{l|}{\textbf{Dataset}}     & \textbf{\# Train} & \textbf{\# Test} \\ 
\hline
\multirow{2}{*}{TIS}     & ToTTo & 20,244    & 1,283    \\
                         & HiTab & 6,943     & 1,254    \\ \hline
\multirow{2}{*}{TIS+TSU} & ToTTo & 20,054    & 1,267    \\
                         & HiTab & 6,864     & 1,215    \\ \hline
\multirow{2}{*}{TIS+PRT} & ToTTo & 0        & 1,217    \\
                         & HiTab & 0        & 1,139    \\ \hline
\multicolumn{2}{l|}{Total}       & 54,105    & 7,375    \\
\bottomrule
\end{tabular}
\caption{Data statistics of TabIS. \label{tab:statistic}}
\end{threeparttable}
\end{table}

\renewcommand{\arraystretch}{1.4} %控制行高
\begin{table}[t]\centering
\setlength\tabcolsep{6pt}
\fontsize{10}{10}\selectfont
\begin{threeparttable}
\begin{tabular}{l|cc|cc}
\toprule
   & \textbf{T-TIS} & \textbf{Ratio} & \textbf{H-TIS} & \textbf{Ratio} \\
\hline
MI & 433                & 33.7\%         & 345                & 27.5\%         \\
MO & 495                & 38.6\%         & 366                & 29.2\%         \\
EJ & 267                & 20.8\%         & 438                & 34.9\%         \\
HA & 88                 & 6.9\%          & 105                & 8.4\%  \\
\bottomrule
\end{tabular}
\caption{Statistics of Option generation strategies used in TIS datasets. "T" and "H" denote "ToTTo" and "HiTab", respectively. \label{tab:stat_opt}}
\end{threeparttable}
\end{table}


Table \ref{tab:statistic} illustrates the data statistics of the datasets used in our experiments. We engage 10 sophisticated annotators to meticulously review and revise the challenging cases (detailed in Section \ref{sec:sis_option_generation}). Out of 410 reviewed samples, the options for 193 samples are manually adjusted.

We employ an expert to assess the data quality on 50 samples each from ToTTo-TTG and HiTab-TTG. The agreement rate on ToTTo-TTG and HiTab-TTG is 94\% and 92\%, respectively, demonstrating the high quality of the proposed TabIS.\TODO{前后两段的准确率差别太大，需要进行更详细的说明，比如第一段说的数据是难数据，占比很小。 aggrement rate是什么，直接就是 accuracy？这两个数字可以直接放到表里}
